Multi-Task Time Series Analysis applied to Drug Response Modelling

Time series models such as dynamical systems are frequently fitted to a cohort of data, ignoring variation between individual entities such as patients. In this paper we show how these models can be personalised to an individual level while retaining statistical power, via use of multi-task learning (MTL). To our knowledge this is a novel development of MTL which applies to time series both with and without control inputs. The modelling framework is demonstrated on a physiological drug response problem which results in improved predictive accuracy and uncertainty estimation over existing state-of-the-art models.

==> tikz/3CM.tex <==
\begin{figure}[t!]
\centering
\scalebox{0.85}{

%\begin{tikzpicture}
%\draw (0,0) --(1,2);
%\end{tikzpicture}
\iftrue
\begin{tikzpicture}[customsq/.style={minimum size=40pt,draw},
                    latentdiscrete/.style={minimum size=30pt,draw},
                    visiblects/.style={circle,minimum size=30pt,fill=purplevis!50, draw},
                    visiblediscrete/.style={minimum size=30pt,fill=purplevis!50, draw},
                    invis/.style={minimum size=0pt,fill=white, inner sep=0pt}]
\definecolor{purplevis}{RGB}{185,164,219}


\node [customsq]  (b3) at (-1.5, 0) {$C_3$};
\node [customsq]  (b1) at (1, 0) {$C_1$};
\node [customsq]  (b2) at (3.5, 0) {$C_2$};
\node [invis]     (control_in) at (1,1.7) {};
\node [invis]     (b0) at (1, -1.5) {};


\draw [thick,->] (b3) to [out=335,in=205] (b1);
\draw[thick, ->] (b1) to [out=155,in=25] (b3);
\draw[thick, ->] (b1) to [out=25,in=155] (b2);
\draw[thick, ->] (b2) to [out=205,in=335] (b1);

% annotations
\draw[thick, ->] (control_in) to [out=270,in=90] (b1);
%\draw[thick, ->] (b1) to [out=270, in=90] (b3);
%\draw[thick, ->] (b1) to [out=270, in=90] (b2);
\node [invis] (control_text) at (1.2, 1.3) {$\omega$};
\draw[thick, ->] (b1) to [out=270, in=90] (b0);

\node [invis] (control_text) at (1.1, -1.1) [right] {$k_{10}$};
\node [invis] (control_text) at (-0.4, 0.8) [right] {$k_{13}$};
\node [invis] (control_text) at (-0.4, -0.8) [right] {$k_{31}$};
\node [invis] (control_text) at (2.0, 0.8) [right] {$k_{12}$};
\node [invis] (control_text) at (2.0, -0.8) [right] {$k_{21}$};
\end{tikzpicture}
\fi
}
\caption{A three-compartment model for Propofol pharmacokinetics.}
\label{fig:3CM}
\end{figure}
